Position Heaps for Parameterized Strings

We propose a new indexing structure for parameterized strings, called parameterized position heap. Parameterized position heap is applicable for parameterized pattern matching problem, where the pattern matches a substring of the text if there exists a bijective mapping from the symbols of the pattern to the symbols of the substring. We propose an online construction algorithm of parameterized position heap of a text and show that our algorithm runs in linear time with respect to the text size. We also show that by using parameterized position heap, we can find all occurrences of a pattern in the text in linear time with respect to the product of the pattern size and the alphabet size.

==> docs/ph_algo.tex <==
%#! platex main
\begin{algorithm2e}[!ht]
\label{alg:ph_algo}
\KwIn{A string $t[1:n]$ }
\KwOut{A position heap $\ph{t}$}
\SetKwData{CURRENT}{currentNode}
\SetKwData{NEXT}{nextNode}
\SetKwData{ROOT}{root}
\SetKwData{UNDEFINED}{undefined}
\SetKwData{LAST}{lastCreateNode}
create $\ROOT$ and $\perp$ nodes\;
$\sufp{\ROOT} = \perp$\;
for each character $c$ create edge $(\perp,c,\ROOT)$\; 
$\CURRENT = \ROOT$\;
$s = 1$\;
\For{$i=1$ to $n$}{
	$\LAST = \UNDEFINED$\;
	\While{not exist edge $(\CURRENT,t[i],\NEXT)$}{
		create node $t[s..i]$\;
		create edge $(\CURRENT,t[i],t[s..i])$\;
		\If{$\LAST\ != \UNDEFINED$}{
			$\sufp{\LAST} = t[s..i]$\;
		}
		$\LAST = t[s..i]$\;
		$\CURRENT = \sufp{\CURRENT}$\;
		$s = s+1$\;
	}
	$\CURRENT = \NEXT$\;
	\If{$\LAST\ != \UNDEFINED$}{
		$\sufp{\LAST} = \CURRENT$\;
	}
}

\caption{Position heap on-line construction algorithm}
\end{algorithm2e}

